Byzantine Fault-Tolerance in Federated Local SGD under 2f-Redundancy

We consider the problem of Byzantine fault-tolerance in federated machine learning. In this problem, the system comprises multiple agents each with local data, and a trusted centralized coordinator. In fault-free setting, the agents collaborate with the coordinator to find a minimizer of the aggregate of their local cost functions defined over their local data. We consider a scenario where some agents ($f$ out of $N$) are Byzantine faulty. Such agents need not follow a prescribed algorithm correctly, and may communicate arbitrary incorrect information to the coordinator. In the presence of Byzantine agents, a more reasonable goal for the non-faulty agents is to find a minimizer of the aggregate cost function of only the non-faulty agents. This particular goal is commonly referred as exact fault-tolerance. Recent work has shown that exact fault-tolerance is achievable if only if the non-faulty agents satisfy the property of $2f$-redundancy. Now, under this property, techniques are known to impart exact fault-tolerance to the distributed implementation of the classical stochastic gradient-descent (SGD) algorithm. However, we do not know of any such techniques for the federated local SGD algorithm - a more commonly used method for federated machine learning. To address this issue, we propose a novel technique named comparative elimination (CE). We show that, under $2f$-redundancy, the federated local SGD algorithm with CE can indeed obtain exact fault-tolerance in the deterministic setting when the non-faulty agents can accurately compute gradients of their local cost functions. In the general stochastic case, when agents can only compute unbiased noisy estimates of their local gradients, our algorithm achieves approximate fault-tolerance with approximation error proportional to the variance of stochastic gradients and the fraction of Byzantine agents.

==> IEEEbib.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{graphs/IMG_1844.jpeg}}]{Sajad Khodadadian} is a PhD student in the Milton  Stewart  School  of  Industrial  and Systems  Engineering  at  Georgia  Tech. He received his bachelor degree at Sharif University of Technology, in Electrical Engineering and Physics. His  research interests  include Reinforcement Learning Theory and Algorithms, Non-convex Optimization, Stochastic Approximation, and Causality.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{graphs/doan_120x160.jpeg}}]{Thinh T. Doan}  is an Assistant Professor in the
Department of Electrical and Computer Engineering
at Virginia Tech. He obtained his Ph.D. degree at
the University of Illinois, Urbana-Champaign, his
master degree at the University of Oklahoma, and his
bachelor degree at Hanoi University of Science and
Technology, Vietnam, all in Electrical Engineering.
His research interests span on the intersection of
control theory, optimization, machine learning, reinforcement learning, and applied probability theory.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{graphs/10P1000-P7-003.jpeg}}]{Justin Romberg}  is the Schlumberger Professor in the School of Electrical and Computer Engineering at the Georgia Institute of Technology, where he
has been on the faculty since 2006. Dr. Romberg received the B.S.E.E. (1997), M.S. (1999) and Ph.D. (2004) degrees from Rice University in Houston, Texas; in 2010, he was named a Rice University Outstanding Young Engineering Alumnus. From Fall 2003 until Fall 2006, he was a Postdoctoral Scholar in Applied and Computational Mathematics at the California Institute of Technology. His current research interest lie at the intersection of statistical signal processing,
machine learning, optimization, and applied probability
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{graphs/SivaTheja.jpeg}}]{Siva Theja Maguluri} is Fouts Family Early Career Professor and Assistant Professor in the School of Industrial and Systems Engineering at Georgia Tech. He obtained his Ph.D. and MS in ECE as well as MS in Applied Math from UIUC, and B.Tech in Electrical Engineering from IIT Madras. His research interests span the areas of Networks, Control, Optimization, Algorithms, Applied Probability and Reinforcement Learning. He is a recipient of the biennial “Best Publication in Applied Probability” award in 2017, “CTL/BP Junior Faculty Teaching Excellence Award” in 2020 and “Student Recognition of Excellence in Teaching: Class of 1934 CIOS Award” in 2020.
\end{IEEEbiography}

==> generic_ft.tex <==
\section{Sufficient Condition}
\label{sec:suff}
